DeepFlow: A Cross-Stack Pathfinding Framework for Distributed AI Systems

Over the past decade, machine learning model complexity has grown at an extraordinary rate, as has the scale of the systems training such large models. However there is an alarmingly low hardware utilization (5-20%) in large scale AI systems. The low system utilization is a cumulative effect of minor losses across different layers of the stack, exacerbated by the disconnect between engineers designing different layers spanning across different industries. We propose CrossFlow, a novel framework that enables cross-layer analysis all the way from the technology layer to the algorithmic layer. We also propose DeepFlow (built on top of CrossFlow using machine learning techniques) to automate the design space exploration and co-optimization across different layers of the stack. We have validated CrossFlow accuracy with distributed training on real commercial hardware and showcase several DeepFlow case studies demonstrating pitfalls of not optimizing across the technology-hardware-software stack for what is likely, the most important workload driving large development investments in all aspects of computing stack.

==> case-old.tex <==
%\input{figs/case-core}
%\input{figs/case-network}
%\input{figs/case-mem}
%\input{figs/case-core-net}


\section{Case Studies}
Here we will show how we use our model to project the impact of logic, network and memory technology scaling on overall performance. 
\name is a very expressive model that not only can be used to predict performance but also to predict hardware counters (number of accesses to different levels of memory hierarchy for different operations, number of bytes transferred for each operation under each parallelism strategy, etc.) which we use to understand the observed pattern.  

\subsection{Methodology}
For all the experiments below we are assuming a system with 512 GPU nodes which can be used to parallelize a model in $35$ different ways.
For example, $64$ GPUs can be used to exploit 64-way data-parallel (\texttt{R1\_C1\_D64\_L1}) strategy, 
or can be used to get 8-way data-parallel and for each data shard use 8-way model parallel strategy (\texttt{CR8\_D8\_L1}).

One thing to note here is that not all parallelism strategies are feasible under a given design configuration (memory capacity limit). 
Different parallelism strategies have different memory capacity requirements per data shard per model shards.
Parallelism strategies with no bars refers to infeasible cases (Figure~\ref{fig:case-core}, \ref{fig:case-net} and \ref{fig:case:case-mem}).

\subsection{Logic Technology Scaling}
As technology node scales down, the number of cores on chip grows which results in improved computational throughput. 
Similarly, cache bandwidth and cache capacity at different levels of memory hierarchy improve. 
Overall, the expectation is to see a large performance improvement from one technology node to the next. 
Figure~\ref{fig:case-core} shows the impact of technology scaling on overall performance across different parallelism strategies.
Contrary to the common belief, the technology scaling shows a negligible improvement in performance.
We use \name to find the sources of bottleneck. Our analysis suggests that execution time is mostly dominated by the data transfer time for the reduction operation which is abundant in parallelism strategies which does not scale with technology nodes. Therefore, we conclude technology scaling would not be sufficient if network technology does not scale hand-in-hand. Indeed, without network technology scaling, it seems techniques as simple as changing parallelism strategies would have more prominent impact on performance than technology scaling. Next we show how improving network technology along with technology scaling can improve performance.

\subsection{Network Scaling}
Next, we study the overall impact of network technology scaling on performance and then see how technology scaling would be different in presence of improved interconnection network.
As shown in Figure~\ref{fig:case-net} network bandwidth improvement has a significant impact on overall performance. For better visibility, we are only showing the feasible parallelism strategies. Note here that the network values refer to the peer-2-peer bandwidth between GPUs and not the aggregate bandwidth. 
Today, we are at 50 GB/s between two GPUs given technologies like NVlink. However, we can see that there is room for performance improvement if we can scale network bandwidth to 400 GB/s. Beyond that, we would see a diminishing return because . 

Figure~\ref{fig:case-core-net} shows the impact of logic technology scaling on performance if interconnection bandwidth would have been 30$\times$ faster than today's SOTA technology (1395 GB/s vs. 48 GB/s).
Unlike Figure~\ref{fig:case-core}, we see a clear trend of performance improvement while improving technology nodes. With interconnection bandwidth bottleneck alleviated, the performance is more or less bottlenecked on core and memory throughput and so we see clear improvement transitioning from technology node 14 to 10 to even 5 nm, but beyond that we see a diminishing return as memory bandwidth would become a new bottleneck.


%case_study/perf_model/energy_per_flop/
\subsection{Memory Technology Scaling} As memory technology improves, we will have more memory capacity and more memory bandwidth at hand. However, our analysis suggests that memory scaling will not improve performance per parallelism strategy but still results in dramatic performance improvements ($8 \times$) as it unlocks new parallelism strategies that were dimmed infeasible before due to memory capacity constraints. Within the realm of feasible parallelism strategies, improving memory bandwidth does not result in any performance improvement as the computation part of the problem is bounded on L2 cache bandwidth. 

%case_study/perf_model/energy_per_membit/


\subsection{Architecture Design Space Exploration}
So far, we studied cases where the hardware configuration is assumed fixed and we explore the impact of technology, network and bandwidth scaling on overall performance. In this subsection, we assume the underlying hardware architecture can also change as we explore the impact of other parameters.
There are many studies that can be conducted having a design space exploration framework. Due to space limitation, we showcase only one such use case.
%
Specifically, we are trying to answer the question of whether or not technology node scaling could be successful assuming we re-design the hardware architecture as we transition to a different technology node -- as is customary. 
Recall from Figure~\ref{fig:core} that technology scaling is not effective if the underlying hardware is fixed.  
We 

==> figs/case-core-net.tex <==
\begin{figure}[htbp]
\centerline{\includegraphics[width=0.95\linewidth]{figs/figs/core-net.pdf}}
\caption{Projecting Logic Technology Advancement Impact on Performance (Interconnection Bandwidth \approx 1.4 TB/s).}
\label{fig:case-core-net}
\end{figure}

==> figs/case-core.tex <==
\begin{figure}[htbp]
\centerline{\includegraphics[width=0.95\linewidth]{figs/figs/core.pdf}}
\caption{Projecting Logic Technology Advancement Impact on Performance (Interconnection bandwidth $\approx$ 48 GB/s).}
\label{fig:case-core-net}
\end{figure}

==> figs/case-mem.tex <==
\begin{figure*}[htbp]
\centerline{\includegraphics[width=0.95\linewidth]{figs/figs/memory.pdf}}
\caption{Projecting Memory Technology Advancement on Performance.}
\label{fig:case-mem}
\end{figure*}

==> figs/case-network.tex <==
\begin{figure}[htbp]
\centerline{\includegraphics[width=0.95\linewidth]{figs/figs/inter_network.pdf}}
\caption{Projecting Network Technology Advancement Impact on Performance.}
\label{fig:case-net}
\end{figure}

==> figs/case.tex <==
%\begin{figure*}[t]
%\minipage{0.45\textwidth}
%  \centerline{\includegraphics[width=0.95\linewidth]{figs/figs/case-tech.png}}
%  \caption{Technology Scaling Exploration: For these experiments, we keep the parallelism fixed at R1-C1-D512-P1 (i.e. only data parallelism), and the hardware template is configured to be similar to a V100 node.}
%  \label{fig:case1}
%\endminipage\hfill
%\minipage{0.45\textwidth}
%  \centerline{\includegraphics[width=0.95\linewidth]{figs/figs/case-all.png}}
%  \caption{Optimizing technology, parallelism and architecture in tandem.}
%  \label{fig:case2}
%\endminipage
%\end{figure*}


%\begin{figure}[!t]
%  \centerline{\includegraphics[width=0.75\linewidth]{figs/figs/case-t%ech.png}}
%  \caption{\textbf{Technology Scaling:} We scale logic technology on the X-axis, top 4 lines show 4 new memory technologies and bottom 3 lines show new network technologies.}
%  \label{fig:case1}
%  \vspace{-0.3cm}
%\end{figure}

%
%\begin{figure}[!t]
%  \centerline{\includegraphics[width=0.75\linewidth]{figs/figs/case-all.png}}
%  \caption{\textbf{Co-optimizing technology, parallelism strategy and hardware architecture design.}} 
%  \label{fig:case2}
%  \vspace{-0cm}
%\end{figure}

\begin{figure*}[htb]
\minipage{0.36\textwidth}
  \centerline{\includegraphics[width=0.9\linewidth]{figs/figs/case-tech.png}}
  \caption{\textbf{Technology Scaling:} scaling logic, memory and network technology}
  \label{fig:case1}
  \vspace{-0.3cm}
\endminipage\hfill
\minipage{0.36\textwidth}
  \centerline{\includegraphics[width=0.9\linewidth]{figs/figs/case-all.png}}
  \caption{Co-optimizing parallelism strategy and hardware architecture design.} 
  \label{fig:case2}
  \vspace{-0.3cm}
\endminipage\hfill
\minipage{0.26\textwidth}
%\centering
%\footnotesize
%\begin{adjustbox}{width=1\textwidth}
%\begin{tabular}{|c|c|}
%\hline
%\#Nodes in Package & Normalized Execution Time \\
%\hline
%1                  & 1                         \\
%\hline
%4                  & 0.802397143               \\
%\hline
%16                 & 0.761674856               \\
%\hline
%64                 & 0.755620015              \\
%\hline
%\end{tabular}
%\end{adjustbox}
\centerline{\includegraphics[width=\linewidth]{figs/figs/Perf_vs_package.png}}
  \caption{Performance improvement from multi-node package} 
  \label{fig:multi-node_package}
%\caption{Best case execution time improvement from multi-node packages}
\endminipage
%\vspace{-0.1cm}
\end{figure*}

==> figs/gemm_p4.tex <==
\begin{figure}[htbp]
\centerline{\includegraphics[width=0.8\linewidth]{figs/figs/p4-val.png}}
\caption{GEMM Validation on Nvidia P4.}
\label{fig:gemm_p4}
\end{figure}
%gemm_val.tex

==> figs/gemm_val.tex <==
\begin{figure}[htbp]
\centerline{\includegraphics[width=0.95\linewidth]{figs/figs/gemm_val_overlay.pdf}}
\caption{GEMM Validation on Nvidia V100.}
\label{fig:gemm_val}
\end{figure}
%gemm_val.tex

==> figs/lm_val.tex <==
\begin{figure}[htbp]
\centerline{\includegraphics[width=0.8\linewidth]{figs/figs/lm_val.pdf}}
\caption{Language Model Validation on V100.}
\label{fig:lm_val}
\end{figure}
%lm_val.tex

==> figs/roofline.tex <==
\begin{figure}[htbp]
\centerline{\includegraphics[width=0.95\linewidth]{figs/figs/dummy.pdf}}
\caption{Hierarchical Roofline.}
\label{fig:hroofline}
\end{figure}

==> hardware_old.tex <==
\section{uArchitecture Generator Engine}
The uArchitecture generator engine, AGE,  takes three sets of inputs: (1) A technology components library, where the characteristics of each component such as cores, different types of memories, network interfaces, etc. are defined, (3) Architecture template, where the overall high-level chip and system organization (such as compute and memory hierarchies) is provided, (2) Hardware resource allocation, where area, power, and chip perimeter budgets are provided for the different components of the system. Using this information, the AGE generates the final uArchitecture parameters (such as overall compute throughput, memory bandwidths at different memory levels, network bandwidth) as shown in Figure~\ref{fig:overview}. 

%In this section, we will first provide details of each of the three inputs and then describe how the uArchitecture generator engine uses these inputs to generate the final uArchitectural parameters of the system.

\subsection{Technology Components Library}

A system is generally composed of many primitive components or building blocks such as the compute units, SRAM banks, DRAM, interconnect network components (on-chip and off-chip), etc. A library of these components and their associated technology parameters are provided as input to the tool through a $tech\_config$ YAML file. We classify these components into three primary categories: compute, memory and network. 
%Next we describe the different hardware attributes we assign to the components in each category.
%\vspace{-0.1in}
\paragraph{Compute}  
Attributes for the minimal compute components such as matrix-multiplier units, vector-matrix multiply units, or a dataflow architecture unit are specified under this category. When a compute component is added to the library, the compute attributes listed in Table~\ref{tab:component-parameter} will have to be defined for that component. The tool user can add any type of compute component in the library ranging from a simple scalar unit to a complex unit comprising of a bundle of tensor cores and capture the micro-architectural characteristics in the final architecture template file.
%\vspace{-0.1in}
\paragraph{Memory}
The memory components in a system can be built out of different technologies (e.g., SRAM, DRAM, MRAM, RRAM, 3D-XPoint). Also, these memory components can be used in two ways: on-chip memory and off-chip memory. A library of fine-grained memory components can be created and stored under this category which is utilized to construct different levels of the memory hierarchy. The characteristics of the on-chip components are described at the granularity of a bank because the smallest on-chip memory unit available to a system designer is usually a memory bank. The parameters of a memory bank such as capacity, bit area, periphery overhead etc. are taken as inputs. 
On the other hand, we model the off-chip memory components such as DRAM, 3D-XPoint, etc., at device level granularity, e.g., an HBM stack. This is because the off-chip components are usually obtained at a device level granularity. For off-chip memories, other parameters such as memory controller area, I/O bus width per device, etc. need to be defined. This information is then used to precisely model the capacity and throughput of different levels of the memory hierarchy under the given area and power constraints.
%\vspace{-0.1in}
\paragraph{Network}
The inter-chip network component is  either intra-node or inter-node communication link. In the case of a multi-chip module (MCM) where multiple compute dies and memory devices are integrated on a 2.5D integration substrate within the same package, the inter-die communication is done using high density and energy-efficient links on the 2.5D substrate. These links are considered as intra-node links. On the other hand, the off-package communication links between nodes are considered as inter-node links. The attributes that need to be defined for inter and intra-die communication network components are provided in Table~\ref{tab:component-parameter}. In case of a waferscale system, the entire wafer could be considered as a single node.


\begin{table}[]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{|c|l|l|}
\hline
\multirow{4}{*}{\textbf{Compute}} & Technology Node & Nominal Area \\ \cline{2-3} 
 & Nominal Voltage & Threshold Voltage \\ \cline{2-3} 
 & Nominal Frequency & Min \& Max Voltage \\ \cline{2-3} 
 & Nominal OP rate & Min \& Max Voltage \\ \hline
\multirow{4}{*}{\textbf{On-chip Memory}} & Technology & Latency \\ \cline{2-3} 
 & Dynamic energy per bit & Static energy per bit \\ \cline{2-3} 
 & Area per bit and total area overhead & Bank Capacity \\ \cline{2-3} 
 & Controller area overhead per bank & Controller power overhead per bank \\ \hline
\multirow{6}{*}{\textbf{Off-chip Memory}} & Technology & Number of links per device \\ \cline{2-3} 
 & Dynamic energy per bit & Nominal Voltage \\ \cline{2-3} 
 & Static power per bit & Nominal Frequency \\ \cline{2-3} 
 & Device Capacity & Minimum Voltage \\ \cline{2-3} 
 & Device Area & Maximum Voltage \\ \cline{2-3} 
 & Memory Controller and I/O Area & Access Latency \\ \hline
\multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Network (intra-node \\      and inter-node)\end{tabular}}} & Nominal Voltage & Number of links per mm \\ \cline{2-3} 
 & Nominal Frequency & Threshold Voltage \\ \cline{2-3} 
 & Nominal Energy per Link & Minimum Voltage \\ \cline{2-3} 
 & Nominal Area per Link & Link Latency \\ \hline
\end{tabular}%
}
\caption{Different technology components.} \label{tab:component-parameter}
\vspace{-0.2cm}
\end{table}



\ignore{
\begin{table}[]
\tiny
\centering
\caption{Different architectural components and their associated technology parameters.}
\label{tab:component-parameter}
\resizebox{\linewidth}{!}{%
\begin{tabular}{|c|l|}
\hline
\multirow{9}{*}{\textbf{Compute}} & Technology Node \\ \cline{2-2} 
 & Nominal Voltage \\ \cline{2-2} 
 & Nominal Frequency \\ \cline{2-2} 
 & Nominal Flop rate \\ \cline{2-2} 
 & Nominal Power \\ \cline{2-2} 
 & Nominal Area \\ \cline{2-2} 
 & Threshold Voltage \\ \cline{2-2} 
 & Minimum Voltage \\ \cline{2-2} 
 & Maximum Voltage \\ \hline
\multirow{9}{*}{\textbf{On-chip Memory}} & Technology \\ \cline{2-2} 
 & Dynamic energy per bit \\ \cline{2-2} 
 & Static power per bit \\ \cline{2-2} 
 & Area per bit \\ \cline{2-2} 
 & Bank capacity \\ \cline{2-2} 
 & Area overhead \\ \cline{2-2} 
 & Controller area overhead per bank \\ \cline{2-2} 
 & Controller power overhead per bank \\ \cline{2-2} 
 & Latency \\ \hline
\multirow{12}{*}{\textbf{Off-chip Memory}} & Technology \\ \cline{2-2} 
 & Dynamic energy per bit \\ \cline{2-2} 
 & Static power per bit \\ \cline{2-2} 
 & Device Capacity \\ \cline{2-2} 
 & Device Area \\ \cline{2-2} 
 & Memory Controller and I/O Area \\ \cline{2-2} 
 & Number of links per device \\ \cline{2-2} 
 & Nominal Voltage \\ \cline{2-2} 
 & Nominal Frequency \\ \cline{2-2} 
 & Minimum Voltage \\ \cline{2-2} 
 & Maximum Voltage \\ \cline{2-2} 
 & Access Latency \\ \hline
\multirow{8}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Network (intra-node \\      and inter-node)\end{tabular}}} & Nominal Voltage \\ \cline{2-2} 
 & Nominal Frequency \\ \cline{2-2} 
 & Nominal Energy per Link \\ \cline{2-2} 
 & Nominal Area per Link \\ \cline{2-2} 
 & Number of links per mm \\ \cline{2-2} 
 & Threshold Voltage \\ \cline{2-2} 
 & Minimum Voltage \\ \cline{2-2} 
 & Link Latency \\ \hline
\end{tabular}%
}
\end{table}






\begin{table*}[h!]
    \centering
   \begin{tabular}{|>{\centering\arraybackslash}m{3cm}|>{\centering\arraybackslash}m{14cm}|}
         \hline
         \multicolumn{2}{|c|}{\textbf{Compute}} \\
         \hline
         \textbf{Technology Node} & The technology node in which the core is implemented \\
         \hline
         \textbf{Nominal Voltage} & The nominal voltage of operation corresponding to the technology node \\
         \hline
         \textbf{Nominal Frequency} & The frequency at which the core can be run when operating at nominal voltage. This number would usually be obtained from a synthesis tool or silicon implementation \\
         \hline
         \textbf{Nominal OP rate} & Number of operation the compute element performs per cycle. E.g., V100 tensor cores performs 128 operations per cycle \\
         \hline
         \textbf{Nominal Power} & The power of the core when run at nominal voltage and frequency \\
         \hline
         \textbf{Nominal Area} & The area of the core implemented in the technology node at the nominal voltage and frequency \\
         \hline
         \textbf{Threshold Voltage} & Transistor threshold voltage ($V_{th}$) for the core. This is used in the voltage and frequency scaling models \\
         \hline
         \textbf{Minimum Voltage} & The minimum voltage at which the core can operate reliably \\
         \hline
         \textbf{Maximum Voltage} & The maximum voltage at which the core can operate reliably \\
         \hline
         \multicolumn{2}{|c|}{\textbf{On-chip Memory}} \\
         \hline
         \textbf{Technology} & The technology of the memory component \\
         \hline
         \textbf{Dynamic energy per bit} & The average energy per bit of access to the memory component \\
         \hline
         \textbf{Static power per bit} & The leakage power per bit \\
         \hline
         \textbf{Area per bit} & The area of a single bit of on-chip memories \\
         \hline
         \textbf{Bank capacity} & The number of bits in a bank of this memory component \\
         \hline
         \textbf{Area overhead} & The area overhead of the peripheral circuitry per bank of this memory component \\
         \hline
         \textbf{Controller area overhead per bank} & The area of the control circuitry per bank. We assume that multiple banks share a control unit (bank select, crossbar interconnect, arbiters etc.) and the overhead grows with the number of banks. For our experiments, we obtain number from ORION2.0~\cite{} \\
         \hline
         \textbf{Controller power overhead per bank} & Similar to the area overhead, we account for the controller's power overhead as well \\
         \hline
         \textbf{Latency} & Average time to access for reads and writes. In our experiments, we calculated this number from CACTI6.0~\cite{} \\
         \hline
         \multicolumn{2}{|c|}{\textbf{Off-chip Memory}} \\
         \hline
         \textbf{Dynamic energy per bit} & The average energy per bit of access of an off-chip memory component is defined here. This includes accessing the memory array and energy to transfer the data, address and commands between the processor and the memory device \\
         \hline
         \textbf{Static power per bit} &  The static power consumed per bit by the memory component. For DRAMs, this is often determined by the average refresh power \\
         \hline
         \textbf{Device Capacity} & The number of bits in the entire memory component. E.g., for high bandwidth memory (HBM) based systems, this is the capacity per 3D-stacked HBM device \\
         \hline
         \textbf{Device Area} & The area of the device that it consumes on the integration substrate such as interposer~\cite{} or waferscale substrate~\cite{}. Therefore, only tightly integrated memory solutions such as HBM's area need to be accounted for in this case \\
         \hline
         \textbf{Memory Controller and I/O Area} & The area overhead of the memory controller and the I/O PHY circuitry on the compute chip per device \\ 
         \hline
         \textbf{Number of links per device} & The width of the data bus connecting the compute die and the memory device \\
         \hline
         \textbf{Nominal Voltage} & The nominal voltage at which the device is operated \\
         \hline
         \textbf{Nominal Frequency} & The frequency of the data bus \\
         \hline
         \textbf{Minimum Voltage} & The minimum voltage at which the device can operate reliably \\
         \hline
         \textbf{Maximum Voltage} & The maximum voltage at which the device can operate reliably \\
         \hline
         \textbf{Access Latency} & Average latency of accessing the memory device \\
         \hline
         \multicolumn{2}{|c|}{\textbf{Network (intra-node and inter-node)}} \\
         \hline
         \textbf{Nominal Voltage} & The nominal voltage at which the inter-chip interconnects operate \\
         \hline
         \textbf{Nominal Frequency} & The nominal frequency at which the inter-chip interconnects operate \\
         \textbf{Nominal Energy per Link} & The energy per bit of the interconnect when operating at nominal voltage and frequency \\
         \hline
         \textbf{Nominal Area per Link} & The amount of area the I/O transceiver circuitry consumes per I/O link \\
         \hline
         \textbf{Number of links per mm} & The number of inter-chip links that the interconnect substrate can accommodate per mm of die edge \\
         \hline
         \textbf{Threshold Voltage} & Transistor threshold voltage ($V_{th}$) for the I/O transceiver circuitry. This is used in the voltage and frequency scaling models \\
         \hline
         \textbf{Minimum Voltage} & The minimum voltage at which the transceiver circuitry can operate reliably \\
         \hline
         \textbf{Link Latency} & The latency to communicate between two chips (includes the router latency)\\
         \hline
         
         
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table*}

}


\input{figs/hardware-system-overview}
\subsection{Architecture Template}
Once all  system components are instantiated from the technology library, the next step is to hierarchically organize one or multiple components from each category to construct the overall system.  Distributed machine learning training is done on scale-out multi-node system, as shown in Figure~\ref{fig:hardware-system-overview}. Such a system consists of multiple individually packaged nodes which communicate through off-package interconnects (such as NVLink, Infiniband etc.) that form the inter-node network. Inside each package, there can be multiple different accelerator nodes connected using an intra-node network. Each accelerator within the package typically consists of one accelerator die that is connected to its own off-chip main memory components (such as HBM, as shown in the figure). Each accelerator die itself can be composed of smaller compute units.

\name  provides a rich template that can be used to specify the overall architectural organization of such an accelerator system. 
%The template is used to specify the high-level micro-architectural organization of the compute units, organization of the memory hierarchy, inter-chip network topology (both intra- and inter- node) and the system hierarchy. 
Next we describe in detail how the template is organized and how different system configurations can be achieved using this template.

\paragraph{\textbf{Compute unit}} As shown in the accelerator die architecture in Figure~\ref{fig:hardware-system-overview}, compute units are often organized in hierarchies. E.g., in an NVIDIA GPU, multiple tensor cores are bundled in a streaming multi-processor (SM) and the SM as a whole interacts with the cache hierarchy. In \name one can express such hierarchy by defining \textit{minimal compute units (MCUs)} and
\textit{MCU bundle}. MCU is the smallest compute unit that we expose to the tool user.  It defines the dataflow model and layout (e.g. MCU can be a systolic array that its height and width are configurable as input). Meanwhile, MCU bundle defines the number of MCUs that are bundled together and are exposed to the first level of memory hierarchy. 

In dataflow architectures such as Eyeriss, TPU etc., data can flow directly between different cores. Hence, the tool allows one to define the type of dataflow within a MCU bundle. Currently the performance model supports three types of dataflow: \textit{weight stationary, activation stationary and output stationary}. The tool can also find the best dataflow strategy among the three for any given kernel.% if the dataflow mode is selected as `best'.

Software runtime, scheduling overheads and the architecture of the cores often restrict the maximum compute utilization. For example, the tensor-cores in NVIDIA V100 incurs fill-drain related under-utilization during tensor loading from the registers and therefore achieves a maximum utilization of 85\%. To account for such overheads, a maximum utilization value can be defined which derates the core throughput by that factor. 

\paragraph{\textbf{Memory Hierarchy and Scope}} The memory hierarchy is defined by initializing multiple memory levels from the highest to the lowest level (i.e., registers to the main memory) as shown in Figure~\ref{fig:hardware-system-overview}. Each level of memory has two attributes: (1) \underline{Memory technology} component from the technology component library which defines the physical attributes of the memory as outlined in Table~\ref{tab:component-parameter}, and (2) \underline{Scope} defines 
the set of components from the next level of memory hierarchy that are accessible from this level of memory hierarchy.
%which micro-architectural components can access that level of memory. 
For example, the `global' scope indicates that the memory level is accessible to all the instances of the higher memory levels.

\paragraph{\textbf{Network Topology}} In \name, we support two levels of network hierarchy: intra-package and inter-package. For each level, a different topology (e.g. mesh, torus, crossbar) can be defined. 


\subsection{Hardware Resource Allocation}
 %
 Hardware design under a limited area and power budget is a fine art of finding the right balance (breakdown of resources) across different u-architectural components. 
 %
 The area and power allocation (and for some components perimeter) of each u-architectural component derives the design and specification of that component. 
 %
We define resource distribution across different components of the compute chip as input parameters, where resource can be area, power and perimeter of the compute chip.  
%
The input definition includes the total area and power budgets for the entire compute node. The total perimeter is inferred from area. 
%
The area budget is usually dictated by packaging constraints. For example, if the compute and memory dies are assembled on a 2.5D silicon interposer-based interconnect substrate, the total area of the node will be limited by the maximum size of the interconnect substrate that can be fabricated. 
%
Compare this to a waferscale system which houses an entire node on a wafer where the total area budget can be as large as 70,000 $mm^2$. 
A node's power budget is determined by the cooling infrastructure that extract heat from the node and the power delivery constraints.

We define budget distribution across different components of the compute graph as a percentage breakdown.
As shown in the YAML snippet below,
%Figure~\ref{fig:area-breakdown}, 
fractions of the total area is distributed across cores, levels of memory hierarchy and network
components. Similarly, the fraction of the compute chip's power and perimeter gets devoted to different hardware components.
%\begin{figure}
\begin{minted}[
    breaklines,
    frame=single,
    fontsize=\tiny
  ]{yaml}
area_breakdown:
    node_area_budget: 1230 #mm2
    proc_chip_area_budget: 815 #mm2
    core: 0.35
    L2: 0.14
    L1: 0.1 
    L0: 0.2
    DRAM: 0.05
    network:
      intra_package: 0.06
      inter_package: 0.1
\end{minted}
%\caption{Example showing area budget allocation and breakdown among different components}
%\label{fig:area-breakdown}
\vspace{-0.3cm}
%\end{figure}

Given the overall resource allocation and distribution, the AGE performs a series of optimizations (voltage-frequency scaling) to find an optimal parameter settings for each u-architectural component. An optimal parameter setting is one that utilizes the most of the allocated budget. Note that an unbalanced resource allocation may leave some of the budget under-utilized. While we allow users to provide a manual breakdown of resources as input, we highly recommend to use SOE (Search and Optimization Engine) to find the best setting which maximizes the overall resource utilization. 
%then calculates the micro-architectural parameters of various chip components which would be used by the PPR for performance prediction. 
%Examples of such output parameters include compute throughput, capacity and bandwidth to the different memory levels and the intra- and inter-node network bandwidths. 

%Often at early stages of an accelerator design, designers have a rough idea of resource budget for each u-architectural component but not necessarily the final parameters.
%This stage mimics the real-world process of hardware design.
%Next, we elaborate the micro-architectural paramter generation for each of these components in detail.

%optimally allocate resources corresponding to each component provided in the architecture template. 
%Besides, the perimeter of the compute die determines the total number of wires that can escape out of the compute chip. Hence, the tool also takes as input the breakdown of the perimeter of the compute die to allocate portions of die perimeter to different off-chip links such as off-chip memory links, intra-node and inter-node links.

\subsection{uArchitectural Parameter Generation}
%\textcolor{blue}{Can we potentially move this to appendix if crunch for space?}
Given the architecture template, the resource breakdown across different components and the technology parameters, we use AGE to find the micro-architectural specification for each architectural component. 
We find the maximum number of minimal compute units that can fit in the given area budget and find the voltage-frequency points to maximize compute throughput under the power budget. 
Similarly, for on-chip caches, we find the memory capacity and memory bandwidth at each level that can fit in the area budget while taking the network and controller overhead into account. For off-chip memories and network interfaces, we use the energy per bit information alongside the PHY area, bump pitch as well as interconnect wiring pitch to determine the maximum bandwidth that can be realized on the chip.

These architectural parameters, throughput, bandwidth and capacity are then provided as input to the performance prediction engine. More details about how we model and calculate these parameters have been explained in Appendix~\ref{detailed_uarch}

\ignore{

\paragraph{Core} For deep learning models, the kernels are usually highly parallel in nature and therefore, our goal is to maximize total compute throughput under the area and power budgets allocated for compute. Given the area budget, we first compute the maximum number of MCUs (minimal compute units) that can fit within the area allocated. 
%Then, we compute the voltage and frequency of the compute units such that the total peak power is within the power budget allocated. 
The nominal frequency and voltage for each MCU is an input to the model, therefore the nominal power for each MCU and the entire core can be derived very easily. 
%
If the nominal power exceeds the power budget, we scale down the frequency and voltage. If we hit the minimum voltage limit set in the component description, we reduce the number of MCUs till we satisfy the total power budget allocated to the compute units.
%
This explains a case where the core design is power-bound and not area-bound.

Once we determine the total number of cores and the frequency of operation, we compute the compute throughput by appropriately scaling the nominal flop rate.
\begin{comment}
\begin{equation}
    Throughput = N \times Flop_{nominal} \times {\frac{f_{op}}{f_{nominal}}}
    \label{eqn:compute_throughput}
\end{equation}
where $N$ is the total number of cores, $Flop_{nominal}$ is the nominal flop rate of each core, $f_{nominal}$ is the nominal frequency corresponding to the technology node of the core and $f_{op}$ is the scaled final operating frequency. We use standard Voltage-Frequency-Power scaling methodology~\cite{} to obtain the operating voltage and frequency.
\end{comment}
\vspace{-0.1cm}
\paragraph{Register and Cache Memory} The total area and power budgets allocated to each level of on-chip memory is split between the memory banks and 
the network circuitry that connects the memory banks at each level to u-architectural components at the next level that are under its scope.
%the on-chip network used to communicate between the microarchitectural components under the scope of that level. 
We assume this interconnect to have a crossbar topology. The total number of components under its scope and the number of banks in that memory level determine the area and power overheads of the network. We iteratively determine the total number of  banks possible at each level of memory hierarchy such that the total area of the banks and the network at every level satisfies the area budget allocation. 
Once we determine the number of memory banks, we calculate total static power of all the banks and we allocate the remaining power budget to dynamic access energy. The available dynamic energy budget determines the maximum achievable throughput.

%as shown in Equation~\ref{eqn:throughput_memory}.
\begin{comment}


\begin{equation}
    P_{static} = P_{static-per-bit} \times N_{banks} \times Capacity_{bank}
    \label{eqn:static_power_cache}
\end{equation}

\begin{equation}
    Throughput = \frac {P_{on-chip-mem} - P_{static}}{Energy_{dyn-per-bit}}
    \label{eqn:throughput_memory}
\end{equation}
\end{comment}
\vspace{-0.2cm}
\paragraph{Main Memory} 
Main memory has two major components that collectively control the overall capacity and bandwidth but are housed in two different places. Memory controller which is placed on the compute chip, and the memory devices are placed outside the compute die within the same package.
The area allocation to each component determines the maximum number of memory devices that can be supported, which in turn determines the total memory capacity. Meanwhile power and perimeter allocation dictates the number of links (that can fit along the compute die), and the frequency of each link which collectively determine the overall off-chip memory bandwidth.

%The number of main memory devices that can fit in a node is determined by three factors:(1) Main memory area budget within the node. E.g., in an interposer or multi-chip module setup, the number of memory devices that can be accommodated in a package is determined by the size of the integration substrate available after the compute/processor chip is placed on the substrate; (2) The number of memory controllers that can fit in the area available in the processor chip. (3) The number of memory interfaces/links that can fit along the available perimeter budget of the compute die. Note that this is dictated by the integration technology's interconnect density. In this framework, we assume that the off-chip memory devices would use standard interfaces and therefore the interface width per device would be fixed and is an input to the tool. 
%The maximum number of memory devices is determined by the most limiting of the three above-mentioned factors. Once the maximum number of memory devices is determined, AGE calculates the total capacity based on the capacity per device. The overall throughput then is calculated based on the frequency and the total interface data-bus width, similar to the case of caches.
%Next, the total static power of the off-chip memory subsystem is computed based on the static power per-bit data. Given the off-chip memory power budget and the static power known, the next step is to calculate the total memory bandwidth based on the remaining power budget. To do so, the frequency of operation of the memory is calculated using the standard voltage-frequency scaling methodology. The overall throughput then is calculated based on the frequency and the total interface data-bus width, similar to Eq.~\ref{eqn:throughput_memory}.


\begin{comment}



%the tool calculates the bus width between the compute and the memory die using Equation~\ref{eqn:bus_width}, where $BusWidth$ is the number of links possible between the compute die and each memory device, $perimeter_dram$ is the perimeter of the compute die that is allocated for off-chip memory communication, $N_{devices}$ is the total number of memory devices, $\#Links_{device}$ is the maximum bus width that each memory device can support and $\#Links_{mm}$ is the total number of inter-chip links that the interconnect substrate can accommodate.

\begin{equation}
\small
\begin{split}
    \#Devices = min(&\frac{Node\ Area - Processor\ Chip\ Area}{Device Area}, \\ & \frac{Area\ budget\ for\ Memory\ Controllers}{Memory\ Controller\ Area},
    \\ & \frac{Perimeter \times \#Links\ per\ mm}{\#Links\ per\ device})
    \label{eqn:num_mem_devices}
\end{split}
\end{equation}
\end{comment}
%Once the bus width per memory device is known, the tool calculates the link frequency based on the main memory budget using the standard voltage-frequency scaling methodology. The tool ensures that the operating voltage satisfies the maximum and the minimum voltage limits set in the technology library. Finally the throughput is calculated similarly as provided in Equation~\ref{eqn:throughput_memory}.
\vspace{-0.2cm}
\paragraph{Network} 
The off-chip network links (intra and inter-package) consume both power and area on the compute die. Moreover, the wires need to escape the periphery of the die which gets determined by the interconnect density and the available chip perimeter. The maximum number of links that can be accommodated in the compute die is limited either by the area available to fit in the link I/O cells or the amount of perimeter available for the links to escape the die periphery. Therefore, the tool uses the area per link, the available area budget, wiring density and the die perimeter budget to find the maximum number of links that can fit in the chip. Next, the tool uses the standard voltage-frequency scaling methodology to find the operating point for each link such that the total network related power is within the power budget allocated. The network bandwidth is then calculated by multiplying the total number of links and the operating frequency of each link. We perform this step for the intra-node network and inter-node network separately.
}

==> map.tex <==
\section{Parallelism Strategy Space}~\ref{sec:pss}


==> mechaflow.tex <==
\input{figs/overview}
\section{CrossFlow Framework}
%https://people.eecs.berkeley.edu/~ysshao/assets/papers/shao2015-toppicks.pdf
%
%Overview
%\subsection{Modeling Methodology}
%\subsection{Performance Modeling Engine}
%\subsection{Accelerator Design Engine}
%As an input, ADE gets total power, area and perimeter for the entire system and breakdown across different hardware components as an input from user.
%We find the best hardware deisgn specified power budget and area budget
%\subsection{Node Placement}
%\subsection{Optimization Engine}
%\subsection{Validation}
%\subsection{Limitations/Future Directions}
%The current work only looks at a homogeneous network of accelerators. There are much more opportunity by specializing hardware to each layer. We leave that as a future work.  
Figure~\ref{fig:overview} shows an overview of the CrossFlow framework. CrossFlow needs the following set of inputs: (1) Architecture template of the accelerator node, which includes different components (e.g., compute cores, levels of memory hierarchy model), specification of each component (e.g., throughput of each compute core, number of compute cores sharing a set of register files, dataflow execution model, and characteristics and scope of different levels of memory hierarchy), (2) System level organization in the form of the system graph (e.g., number of accelerators/nodes per package, number of packages in the system, the network topology connecting nodes within a package and across the package), (3) Technology parameter specification of each hardware component (4) Design budgets for accelerator node design (area, power, perimeter) (5) ML model specification in the form of a high-level compute graph, parameters of each compute node (kernel type, tensor dimensions), (6) Parallelism strategy (data, model, kernel, and/or pipeline parallelism dimensions) which distributes the compute graph across the entire system. 

\input{figs/transformation.tex}
Given these inputs, CrossFlow predicts the end-to-end performance of one iteration (i.e., single batch) of the ML model. To do so, CrossFlow breaks the problem into the following phases: (1) uArchitecture generator engine which estimates microarchitecture parameters for the accelerator node under design constraints dictated by technology and resource budget (2) Compute graph transformation engine which replicates the compute graph along different dimensions in the parallelism space and adjust kernel dimensions to reflect the parallelism strategy (3) Device mapping engine which maps compute graph to system graph (4) Compute graph component prediction engine which estimates the time for all the vertices and the edges in the compute graph, and (5) An event-driven simulator to estimate the time to completion of one iteration through the graph, respecting resource scheduling constraints.


%performance prediction engine predicts time foreach node and each edge within the graph individually. Havingtime for each node and each edge within the compute graph, we  will  use  an  event-driven  simulator  that  walks  over  thegraph and triggers new event dictated by data dependency andresource mapping schedule.
\vspace{-0.15in}
\subsection{Compute Graph Transformation and Device Mapping Engine}

%Given the ML model description (in form of a compute graph), the system topology (in form of a system graph) and the parallelization strategy, we use device mapping engine to map the vertices of the compute graph (kernels) onto the vertices of the system graph (nodes) and map the edges of the compute graph (data dependency edges) to the edges of the system graph (physical network links). However, before the mapping happens, we transform the compute graph to reflect the parallelism strategy specified by the user.

Given the ML model description (in form of a compute graph), and the parallelization strategy, we first transform the compute graph to reflect the parallelism strategy. Next, we use device mapping engine to map the vertices of the compute graph (kernels) onto the vertices of the system graph (accelerator nodes) and map the edges of the compute graph (data dependency edges) to the edges of the system graph (physical network links).

\vspace{0.1in}
\textbf{Transformation}
Figure~\ref{fig:transformation} shows an example of graph transformation. Data parallelism, would result in replicating the graph and connecting the corresponding compute vertices in a fashion consistent with the reduction algorithm. For example, in case of ring-all-reduce, the corresponding vertices would be connected in a ring fashion. Note that the new edges that will be added to the graph will be marked as \textit{cross-edge} to capture the fact that they connect compute vertices belonging to different data parallel shards placed on separate devices.
%
Model/kernel parallelism would result in replacing each vertex in the compute graph with sub-vertices and adjusting the problem size for each device and connecting the sub-vertices in a manner consistent with the parallelism strategy and the reduction algorithm.  
Much similar to data parallelism, the new edges would be marked as \textit{cross-edge}.
%
Similarly pipeline parallelism slices the compute graph in to multiple sub-graphs such that each sub-graph could be placed on to a separate device such that the computation across consecutive batches can be pipelined.
%Pipeline parallelism, unlike other forms, does not result in replication or replacement of graph nodes. It simply modifies the edge type between nodes across layers that are mapped to different pipeline stages to capture their cross-connection nature. 

\vspace{0.1in}
\textbf{Mapping}
Depending on the parallelism strategy, the transformed compute graph can take the form of a 5D/4D/3D hypercube. However, the underlying system topology may be a 2D or 3D hypercube. This means that multiple edges in the compute graph would need to be mapped in to one edge/link of the system graph. The number of logical edges that are mapped into a physical edge is an important metric as it captures the effect of link bandwidth sharing which ultimately affects the communication overhead. Based on link sharing, we allocate the derated/partial link bandwidth to the edges of the compute graph. In order to find a mapping that minimizes the maximum number of edges that is mapped in to each network link, we use a greedy heuristic. Our heuristic works as follows: starting with one axis in the parallelization space, we map the vertices along that axis as close as possible, before moving to the vertices in the second axis. We repeat this for different permutations of axes and choose the one which minimizes the communication overhead.

%\todosaptadeep{These different parallelism strategies have major implications on end-to-end performance and stress different resources of the system. As an example, very large models often wouldn't fit in the main memory capacity of a single accelerator device, and therefore model and/or pipeline parallelism needs to be employed. Model parallelism on the other hand, can stress inter-node network characteristics.}

\subsection{Performance Prediction Engine}
We estimate the end-to-end performance in a hierarchical manner. In the first step, we predict the performance of each kernel on the hardware node that is mapped onto. Having all compute nodes performance in place, we follow an event-driven simulation to capture the end-to-end timing. We explain these two steps in more details.

\subsubsection{Estimation of the Compute Graph Components}

Crossflow uses hierarchical roofline analysis to predict the execution time of each kernels in the transformed compute graph. The edge component, i.e., the inter-device communication overhead is calculated based on a simple throughput model.

\vspace{0.1in}
\textbf{Hierarchical Roofline Model}
Roofline model is an analytical model that relies on accurate estimation of operational intensity (OI) to predict if an application is memory-bound or compute-bound. Once this is known, it uses a simple throughput analysis to estimate timing (\#flops/compute throughput if compute-bound, or \# memory accesses/memory bandwidth if memory-bound).
Hierarchical roofline analysis much similar to roofline analysis relies on operation intensity estimation to measure OI wrt. different levels of memory hierarchy to predict if an application is compute-bound, L1-bound, L2-bound, etc. 
Operational intensity would be different for different levels of memory hierarchy, controlled by the number of accesses to each level. Hence, our performance estimation very much depends on accurate estimation of number of accesses to each levels of memory hierarchy, which in turn depends on the tiling choices at each level. 
%Once the tile sizing and roofline estimations for each level of memory hierarchy is in place, the overall performance is dictated by the slowest performing component. 

\vspace{0.1in}
\textbf{Memory Hierarchy Modeling}
%re-streaming coupled with tiling
%As we pointed out before, the success of roofline analysis very much depends on the accurate estimation of the number of accesses to each level of memory hierarchy. 
The number of accesses to each level of memory hierarchy is a function of the underlying hardware (memory capacity at each level) and the algorithmic implementations (tiling strategies). For each level of memory hierarchy, we explore $N$ different tiling strategies that meets the hardware constraints (memory capacity at that level), where $N$ is a tunable parameter in the framework. 
For an architecture, with $L$ levels of memory hierarchy, this requires searching over the space of $N^L$ tiling combinations. Empirically, we found that for $L=3$, $N \approx 20$ results in a reasonably accurate estimation. 

%For any given tiling strategy, we find the number of times each tile needs to be re-streamed from the next (lower) level of memory hierarchy. We start from the lowest level of memory hierarchy (e.g. L2 cache in the case of a GPU-like architecture) and walk upward to estimate the number of accesses to each level and propagate the re-streaming factor upward. Refer to Alg.~\ref{alg:}. 
%Within each level (say $L_{(i)}$), the number of accesses from the higher-level $L_{(i-1)}$ is dictated by the tiling parameters at the current level ($T_{(i)}$) and the higher level ($T_{(i-1)}$). $T_{(i)}$ itself is a triplet that captures tiling along the input, output and inner dimension at level $i$.

%%%%%%%%
\vspace{0.1in}
\textbf{DataFlow Modeling} 
The number of accesses to each level of memory hierarchy, except for level 0 (i.e. register files) is dictated by the tiling parameters at the current and higher levels. The number of accesses to register file will be determined by the number of instructions executed in the execution engine and the dataflow strategy governing mapping and communication between those engines (e.g. weight stationary ($WS$), activation stationary ($AS$) and output stationary~\cite{eyeriss,timeloop}). 
The execution engine structure dictates how many times a piece of data could be reused internally before accessing the register file. We refer to this number as \textit{reuse factor (K)}.
For example, in the case of an execution engine being a single Fused Multiply Add (FMA), each data element will be reused only once. 
In the case of a 2-D systolic array with size $N_x$ and $N_y$, each data element could be reused $T_x/N_x$ or $T_y/N_y$ or $T_z/N_z$ times, depending on the choice of dataflow strategy and tile size (i.e. $T_x$, $T_y$ and $T_z$).

%We model three different dataflow strategies, weight stationary ($WS$), activation stationary ($AS$) and output stationary ($OS$) and allow users to pick their desired strategy from one of the $\{WS$, $AS$, $OS$, best$\}$ choices. Here, the \textit{best} will selects the best strategy among the three choices.

%We use the following equation to calculate number of accesses to register files:

%\begin{equation*}
%    \#L_0\_accesses = \#Flops \times \frac{N_x.N_y + K. N_x + K. N_y}{2.K.N_x. N_y}
%\end{equation*}

%Where $K$ is the reuse factor whose value is determined by the dataflow strategy (explained above).

\vspace{0.1in}
\textbf{Inter-device Communication Modeling}
%Once the transformed compute graph is mapped down to the system graph, we calculate the number of bytes that needs to be transferred through each edge ($D_e$). On the other hand, 
Compute graph to system graph mapping engine generates the information about logical edge to physical link mapping.  Based on how many edges share a link, we find the portion of the bandwidth of the physical link that is allocated for every edge sharing that link.
For edges which are allocated multi-hop paths, the physical link with the minimum bandwidth allocation becomes the bottleneck. We use the bottleneck bandwidth for each edge to estimate transfer time for that edge.
%( equation~\ref{eqn:bandwidth_derating_factor}). 
%For edges which are allocated multi-hop paths, the physical link with the minimum bandwidth allocation becomes the bottleneck. We then use the bandwidth allocated in the bottleneck link (equation~\ref{eqn:bottleneck_link}) to estimate the total time ($T_e$) taken to transfer the tensors from one device node to the other.

%\begin{equation}
%    \label{eqn:bandwidth_derating_factor}
%    B^l_e = \frac{B^l}{\sum_{e \in E} X^l_e} ~~~~\forall l\in L
%\end{equation}
%\begin{equation}
%    \label{eqn:bottleneck_link}
%    \displaystyle{B_e = \min_{l}(B^l_e)}
%\end{equation}
%\begin{equation}
%    T_e = \frac{D_e}{B_e}
%\end{equation}
%where $X^l_e$ is 1 if edge $e$ is assigned to link $l$, otherwise 0.

%%%%%%%%%%%
\ignore{
\subsection{Parallelism Modeling} 
Once the dataflow strategy is decided, we \textit{transform} our graph to reflect the impact of different forms of parallelism strategies, such as data, model and pipeline parallelism. Figure~\ref{fig:} shows an example of such transformation.

%
Data parallelism would result in replicating the graph and connecting corresponding compute nodes in a fashion consistent with the reduction algorithm. For example, in case of ring-all-reduce, the corresponding nodes would be connected in a ring fashion. Note that the new edges that will be added to the graph will be marked as \textit{cross-edge} to capture the fact that they connect nodes belonging to different accelerators.

%
Model parallelism would result in replacing each compute node with sub-nodes and adjusting the problem size within each node and connecting the sub-components in a manner consistent with the parallelism strategy and the reduction algorithm.  
Much similar to data parallelism, the new edges would be marked as \textit{cross-edge}.

%
Pipeline parallelism, unlike othems, does not result in replication or replacement of graph nodes. It simply modifies the edge type between nodes across layers that are mapped to different pipeline stages to capture their cross-connection nature.  
% 


%%%%%%%%%%%
\vspace{0.1in}
\textbf{Network Modeling} 
So far we discussed how performance prediction engine predicts the time for each node within the compute graph. Here, we look deeply into how to model performance for each edge.
%
Recall that depending on the choice of parallelism strategy, the transformed compute graph can be a 5D/4D/3D hyper-cube (refer to Figure~\ref{fig:}).
%
However, 5D/4D/3D hyper-cube is not realizable in hardware. Physically speaking, the interconnection network across several nodes is usually structured hierarchically. Compute nodes that sit on a wafer are usually connected through one network topology and nodes across wafers are connected through another network topology. 
%
For example Nvidia DGX box consists of 8 GPUs, with one GPU on each wafer and wafers organized in a 3D hyper-cube on a ... substrate. 
%
In this paper, we are interested in wafer-scale integration, hence we study cases where we can fit more than one GPU/accelerator on one wafer. For connecting nodes on one wafer,  we assume a 2D mesh network topology, and for nodes across wafers, we assume a 2-D torus. This is similar to what recent wafer-scale hardware accelerators like Cerebras are adopting.

Note the mismatch between physical and logical network topology (5D/4D/3D vs. 2D). This indicates that multiple edge in logical graph can be mapped into one edge on physical layout. The number of logical edges that are mapped into a physical edge is an important metric as it captures the number of virtual channels required to simulate the connection in logical graph. The number of virtual channels per edge dictates the factor by which we have to derate the physical connection to capture the actual bandwidth. Overall bandwidth is dictated by the slowest link. So our goal is to find an optimal mapping that minimizes the maximum number of edges that is mapped into each edge across all edges. We use greedy heuristics to find such mappings. Our heuristic works as follow: starting with one axis, we try to map the nodes along that axis as close as possible, before moving to elements along the second axis and we repeat this until we map all axes. We repeat this for different permutations of axes. Figure~\ref{fig:} shows an example of a 4D to 2D mapping.
}

%%%%%%%%%%
\subsubsection{End-to-End Time Estimation}\label{subsec:end2end}
%include discussion around pipeline parallelism and 
In prior subsection, we discussed how we start with the original compute graph ($G_0$) and transform it into an extended form ($G_3$) that captures different forms of parallelism strategies that are specified by the user. 
%Each node in the final transformed graph captures a model shard with a data shard. 
%This transformation is necessary to find an accurate estimation of edge timing after physical mapping. 
After the mapping stage, timings for all edges in the transformed graph would be available and after per-component time estimation, timings for all nodes would be available.
Once we have all the timings for all sub-kernels and edges in place, we calculate the end-2-end time by collapsing the transformed graph into its original form. As we move in opposite order, we annotate each node in the compute graph with the updated time. Once the graph is back in its original form ($G_0^'$), the only parallelism strategy that still needs to be taken care of would be pipeline parallelism. 
Once the resource mapping is decided, the overall time measurement would be a matter of graph traversal while respecting the resource constraints.
Here, resources would be compute nodes and communication links.
We assume each resource can be allocated to one node or one edge at a time. Once each edge or node computation is over, it would be back to the resource pool for grab. Overall, pipeline parallelism is simulated in an event-driven manner.



==> par_vs_size.tex <==
Large number of options for compute node exists for programmers. 
Different cloud providers have different hardware. It is hard to figure out which one to go with for distributed training.

Programmers use high level programming libraries and platforms such as TF/Pytorch to implement ML models on these compute nodes. 
Beneath the high level platforms, the hardware manufacturers provides optimized implementation of various ML kernels. As a result the programmers often would not need to spend time and resources in optimizing for the given hardware and would just use the library components to stitch together a model. 

The most common ideology of programming using platforms like TF and PyTorch is that a programmer writes the ML model's DFG. Then based on the amount of memory available per node, the programmers fix the batch size such that all the overall memory requirement is less than that of the memory available in the hardware. Then, if distributed training is needed, programmers often rely on libraries for implementation of data parallelism, model parallelism and/or pipeline parallelism. Examples of such libraries include MeshTF, GPipe, Horovod etc. 

Choosing the right parallelism strategy for a given model and hardware however is not trivial. For example, a hardware node can be a NVIDIA A100 GPU with 320 TFLOPs of compute and 80GB memory or it can be a Cerbras waferscale engine which has XXX PFLOPs of compute and 40GB of memory. Given that the characteristics of the hardware node itself can vary wildly, how to use multiple of these nodes for distributed computing where the inter-node network also plays a big role in determining the overall performance of training is a very challenging task. In this work, we ask the question: can we create simple rules to guide the parallelism strategy in a distributed computing environment which takes in to account the characteristics of the underlying hardware node? 

We also ask the question: Is it worth for system builders to provide larger black-box nodes to programmers and hide away all the details inside the node from programmer? Does that ideology hurt resource utilization in a distributed training environment? What is the right level of granularity that the programmers should be exposed to?

==> removed_text.tex <==
We use hierarchical roofline analysis to predict time for each node within the graph.
To predict performance of an application on a given hardware, roofline model calculates operational intensity (OI) to find if application is memory-bound or compute-bound.
Hierarchical roofline model much like roofline analysis relies on operation intensity estimation to measure performance.
Note here that operational intensity would be different for different levels of memory hierarchy, controlled by the number of accesses to each level. Hence, our performance estimation very much depends on accurate estimation of number of accesses to each levels of memory hierarchy. Once the roofline estimations for each level of memory hierarchy is in place, the overall performance is dictated by the slowest performing component. 

%%%%%%%%%%%
\subsection{Parallelism Modeling} 
Once the parallelism strategy is decided, we \textit{transform} our graph to reflect the impact of different forms of parallelism strategies, such as data, model and pipeline parallelism. Figure~\ref{fig:} shows an example of such transformation.

%
Data parallelism, would results in replicating the graph and connecting corresponding nodes in a fashion consistent with the reduction algorithm. For example, in case of ring-all-reduce, the corresponding nodes would be connected in a ring fashion. Note that the new edges that will be added to the graph will be marked as \textit{cross-edge} to capture the fact that they connect nodes belonging to different accelerators.

%
Model parallelism would results in replacing each node with sub-nodes and adjusting the problem size within each node and connecting the sub-components in a manner consistent with the parallelism strategy and the reduction algorithm.  
Much similar to data parallelism, the new edges would be marked as \textit{cross-edge}.

%
Pipeline parallelism, unlike other forms, does not result in replication or replacement of graph nodes. It simply modifies the edge type between nodes across layers that are mapped to different pipeline stages to capture their cross-connection nature.  
% 


%%%%%%%%%%%
\subsection{Network Modeling} 
So far we discussed how performance prediction engine predicts the time for each node within the compute graph. Here, we look deeply into how to model performance for each edge.
%
Recall that depending on the choice of parallelism strategy, the transformed compute graph can be a 5D/4D/3D hyper-cube (refer to Figure~\ref{fig:}).
%
However, 5D/4D/3D hyper-cube is not realizable in hardware. Physically speaking, the interconnection network across several nodes is usually structured hierarchically. Compute nodes that sit on a wafer are usually connected through one network topology and nodes across wafers are connected through another network topology. 
%
For example Nvidia DGX box consists of 8 GPUs, with one GPU on each wafer and wafers organized in a 3D hyper-cube on a ... substrate. 
%
In this paper, we are interested in wafer-scale integration, hence we study cases where we can fit more than one GPU/accelerator on one wafer. For connecting nodes on one wafer,  we assume a 2D mesh network topology, and for nodes across wafers, we assume a 2-D torus. This is similar to what recent wafer-scale hardware accelerators like Cerebras are adopting.

Note the mismatch between physical and logical network topology (5D/4D/3D vs. 2D). This indicates that multiple edge in logical graph can be mapped into one edge on physical layout. The number of logical edges that are mapped into a physical edge is an important metric as it captures the number of virtual channels required to simulate the connection in logical graph. The number of virtual channels per edge dictates the factor by which we have to derate the physical connection to capture the actual bandwidth. Overall bandwidth is dictated by the slowest link. So our goal is to find an optimal mapping that minimizes the maximum number of edges that is mapped into each edge across all edges. We use greedy heuristics to find such mappings. Our heuristic works as follow: starting with one axis, we try to map the nodes along that axis as close as possible, before moving to elements along the second axis and we repeat this until we map all axes. We repeat this for different permutations of axes. Figure~\ref{fig:} shows an example of a 4D to 2D mapping.
